Towards a Transpiler for C/C++ to Safer Rust

Rust is a multi-paradigm programming language developed by Mozilla that focuses on performance and safety. Rust code is arguably known best for its speed and memory safety, a property essential while developing embedded systems. Thus, it becomes one of the alternatives when developing operating systems for embedded devices. How to convert an existing C++ code base to Rust is also gaining greater attention. In this work, we focus on the process of transpiling C++ code to a Rust codebase in a robust and safe manner. The manual transpilation process is carried out to understand the different constructs of the Rust language and how they correspond to C++ constructs. Based on the learning from the manual transpilation, a transpilation table is created to aid in future transpilation efforts and to develop an automated transpiler. We also studied the existing automated transpilers and identified the problems and inefficiencies they involved. The results of the transpilation process were closely monitored and evaluated, showing improved memory safety without compromising performance and reliability of the resulting codebase. The study concludes with a comprehensive analysis of the findings, an evaluation of the implications for future research, and recommendations for the same in this area.

==> content/intro.tex <==
\section{Introduction}
%\subsection{Rust Language}
%\noindent
% \textit{Rust} is a system programming language that gives you access and fine-grained control over system resources, memory, etc. Anything that we can build with low-level C++ can be built with Rust. 
\textit{Rust} \cite{RustRef1,rustB1} is a systems programming language that provides developers with low-level access and control over system resources such as memory, file systems, and networking. This makes it ideal for building software applications that require performance, efficiency, and reliability, such as databases, compilers, and other low-level systems \cite{RustRef1,10.1145/3158154}.


Rust's notable feature is its absence of a garbage collector, distinguishing it from most other high-level languages. Rust achieves memory safety through its sophisticated type system that tracks variable lifetimes at compile-time. This enables Rust to automatically insert optimized LLVM/assembly instructions for memory deallocation, resulting in improved performance and stability \cite{rustB1}. 
%
%
%One of the unique features of Rust is that it does not have a garbage collector, which is a common feature in other high-level programming languages. This means that Rust automatically manages memory allocation and deallocation to prevent memory leaks. In addition, it also provides complete control over memory allocation and deallocation whenever required, allowing developers to optimize memory usage. All this, in turn, provides a performance boost and improved stability compared to languages with a garbage collector \cite{rustB1}.
%\newline
In addition to its low-level control and performance, the automatic memory allocation and deallocation also makes Rust a memory-safe language, which prevents common programming errors such as null pointer dereference and buffer overflows. This makes it easier for developers to write correct, secure, and reliable code.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.5em}
%\noindent
\subsection{Why migrate to Rust?}
Given these features, it's easy to see why Rust is an attractive option for organizations that need to migrate their existing infrastructure to a new platform. By using Rust, organizations can take advantage of its low-level control, performance, and memory safety to build software that is faster, more efficient, and less prone to errors. Whether you're building a new system from scratch or migrating an existing one, Rust is a powerful tool that can help you achieve your goals.

\remove{
%\newline
%\newline
Rust was initially developed for the Mozilla Firefox browser to handle its memory leaks. However, its efficiency and advantages attracted many C++ developers who began to use Rust instead, commonly for game development.
%\newline
%\newline
}

Rust also has a strong focus on safety and security. The language enforces strict ownership and borrowing rules, making it difficult for developers to write code that can result in undefined behaviour, race conditions, and other security issues. This helps organizations reduce the risk of security vulnerabilities in their software and improve the overall reliability of their systems.
%\newline
%
Another important aspect of Rust is its highly optimized runtime system. The Rust compiler is designed to generate highly efficient machine code, making it a good choice for performance-critical systems. Rust also provides a number of performance-related features such as inline functions and zero-cost abstractions, which can help developers write high-performance code \cite{bugden2022rust} that is both readable and maintainable.
%\newline

In terms of community and support, Rust is a well-established and rapidly growing programming language. The language has a large and active community of developers who contribute to the language and its associated libraries, making it easier for organizations to find resources and support when they need it. Additionally, Rust has a rich ecosystem of libraries and tools that can help organizations quickly and easily build and deploy their systems.
%
Given the range of benefits that Rust offers, it is an excellent choice that can help an organization achieve its goals and succeed in a rapidly changing technological landscape.
%\newline
\remove {
In conclusion, Rust is a powerful, flexible, and secure systems programming language that provides organizations with a range of benefits for building high-performance, reliable, and safe software. Whether you're building a new system from scratch or migrating an existing one, Rust is an excellent choice that can help you achieve your goals and succeed in a rapidly changing technological landscape.
}

 %\sr{Sec 1.1 may be shortened.. seems some points are repeated.. [UPDATED]} 
% \begin{enumerate}
% \item Rust is syntactically similar to C++ but provides memory safety without garbage collection and increased speed.
% \item It gives you low-level access to system resources
% \item Rust specifically is designed to build software where performance and correctness are essential.
% \end{enumerate}
\remove{
\subsection{Migration of Samsung's Tizen operating system code base from C/C++ to Rust}
Rust is specifically designed to build software where performance and correctness are essential. Properties that are essential while developing embedded systems. Thus making it one of the choices while developing embedded devices’ operating systems.
\\
\\
\textit{Samsung Electronics} uses \textit{Tizen} as the operating system on its devices, such as Smartwatches and Smart TVs. Tizen is directly responsible for interacting with the hardware. The organization intends to migrate the existing code base of Tizen from C/C++ to Rust to take advantage of its increased speed and memory safety.
}
\vspace{-0.5em}
\subsection{Problem and Contributions}
%\noindent
Various organizations such as Samsung are looking into Rust. For migration of existing codebases in C++ to Rust, these organizations will not intend to rebuild the existing developed and well-tested modules from scratch. It is thus very much essential to have a trusted auto transpiler for C++ to Rust.  

\textit{Samsung Electronics} uses \textit{Tizen} as the operating system on its devices, such as Smartwatches and Smart TVs. Tizen is directly responsible for interacting with the hardware. As an example C++ codebase for our study, in this work we consider a fragment of the Tizen OS.  


There have been attempts to build transpilers from C/C++ to Rust. One of our contributions is a detailed exploration of the existing auto transpilers. We evaluated several auto transpilers for their ability to transpile code to safe Rust, using both simple programs and a full-scale Tizen's gperf module. Our assessment involved analyzing the generated code for accuracy and reliability, and identifying both positive and negative aspects of each tool. Our findings indicate that the existing transpilers were unable to consistently produce reliable safe Rust code.
%\sr{ADD a couple of lines of summary on this [UPDATED]!!}

\remove{
The project involves collaboration between Samsung R\&D, Bangalore and aims to convert the Tizen platform modules from C++ to Rust in a safe and reliable manner. 
}
%Our study/analysis of the exting transpilers for C++ to Rust showed the need to re
Based on the study of the existing auto transpilers, there is a need to explore further on building a safe and reliable transpiler for C++ to Rust, that led to the following main contributions of this work.

%The ultimate goal of the project is to use an automated transpiler to transpile the codebase, making the process more efficient for future modules.
%\newline


 
In this work, the focus is on understanding the different constructs of Rust and how they correspond to the constructs of C++. A deep dive into the language and its features is conducted, including the correlation between these constructs and how they can be implemented in Rust. For example, we explored how Rust's concept of references and borrowing replaces C++'s raw pointers and null pointers.
%\newline

We then proceeded to manually transpile a module, the gperf module of Tizen platform (originally written in C++), as a proof of concept. This manual process helped us gain a deeper understanding of the language and its constructs. Based on the learning from this process, we have created a transpilation table. 
This transpilation table that resulted will guide future transpilation efforts and also form the basis for the creation of an automated transpiler.


The use of Rust in the Tizen platform is expected to bring increased reliability without compromise on the performance, as Rust is a memory-safe language that provides low-level access to system resources. 
From the module that we have considered in this study, we have also compared and provided some insights on the performance of C++ Vs. Rust.

\remove{
The transpilation process and the resulting codebase will be closely monitored to ensure the desired results are achieved.}


